Learning Strategy-Aware Linear Classifiers

We address the question of repeatedly learning linear classifiers against agents who are strategically trying to game the deployed classifiers, and we use the Stackelberg regret to measure the performance of our algorithms. First, we show that Stackelberg and external regret for the problem of strategic classification are strongly incompatible: i.e., there exist worst-case scenarios, where any sequence of actions providing sublinear external regret might result in linear Stackelberg regret and vice versa. Second, we present a strategy-aware algorithm for minimizing the Stackelberg regret for which we prove nearly matching upper and lower regret bounds. Finally, we provide simulations to complement our theoretical analysis. Our results advance the growing literature of learning from revealed preferences, which has so far focused on "smoother" assumptions from the perspective of the learner and the agents respectively.

==> 5-simulations.tex <==
\section{Simulations with Approximate In-Oracles}\label{sec:sims}

In this section, we present our experimental results\footnote{Our code is publicly available here: \url{https://github.com/charapod/Learning-Strategy-Aware-Linear-Classifiers}}. Since all real, currently available datasets for classification are \emph{not} collected taking the strategic considerations of the agents into account, they \emph{cannot} be used for evaluating our algorithm. Indeed, one cannot be certain whether the currently reported feature vectors stem from an altered original feature vector or not. In order to evaluate empirically $\grinder$'s performance against other algorithms, one needs to know the original feature vectors $\vx_t$. In Appendix~\ref{app:simulations}, we include extra simulations with a different regression oracle, along with an extended discussion both on the setups, and the findings.


\begin{figure}[h!]
\includegraphics[width=\linewidth]{img/discr_comparison_100.png}
\caption{$\grinder$ vs. $\textsc{Exp3}$ for a predefined action set.\label{fig:discr}}
\end{figure}

\paragraph{Simulations Setup.} We fix $d = 2$. To make our model more realistic, and drawing intuition from \citet{drsww18}, we assume that we do not just face strategic agents (called \emph{spammers} with labels $y_t = -1$ and feature vectors drawn from $\vx_t \sim \texttt{Unif}[0.0,0.6]^2$), but also, with probability $p$, agents that do not wish to try and fool us (called \emph{non-spammers} with labels $y_t=1$ and feature vectors drawn from $\vx_t \sim \texttt{Unif}[0.4, 1]^2$). Note than in this case, our theoretical analysis remains unchanged, except for the part that computes the variance of the estimator. The agents best-respond using the following utility function: $$u_t(\alpha, \vz(\alpha;\sigma_t)) = \delta \cdot \1 \{\langle \alpha, \vz(\alpha;\sigma_t) \rangle \geq 0\}\cdot \1 \{\hat{y}_t = y_t\} - \|\vx_t - \vz(\alpha;\sigma_t)\|_2$$for $3$ different values of $\delta: 0.35, 0.7, 1$. We run two big sets of simulations: in the first set of simulations, we assumed a \emph{predefined} action space of size $100$ that both $\grinder$ and $\textsc{Exp3}$ use. In the second one, $\grinder$ is run on a fully continuous interval, and $\textsc{Exp3}$ on a fixed discretization of that interval. Each instance was run for $T = 2000$ timesteps, with $30$ repetitions for each timestep. The solid plots correspond to the \emph{empirical mean} of the regret in the predefined action space simulations, and to the \emph{cumulative loss} in the continuous space ones, while the opaque bands correspond to the $10$th and the $90$th percentile. 

Unless otherwise specified, $\grinder$ is run using an approximation oracle, which uses past spammer data to train a logistic regression model for each $\Pr^{in}[\alpha]$. For the case of the predefined action set, we can compute $\Pr^{in}[\alpha]$ precisely, but this is no longer the case in the continuous action set. We present the results for the predefined action set as a way to measure experimentally the performance of our approximation oracle compared to the precise one. In Appendix~\ref{app:simulations}, we explain thoroughly how the logistic regression is run, and we also present simulation results for another approximation oracle. In summary, we see that both with the use of a precise oracle and with the use of an approximation one for every $\delta$, and for every $p$ our algorithm performs better than $\textsc{Exp3}$. Interestingly, the approximation oracle follows very closely %
 the performance of the precise one.

\begin{figure}[h!]
\includegraphics[width=\linewidth]{img/cont_delta_comparison_100.png}
\caption{$\grinder$ vs. $\textsc{Exp3}$ for a continuous action set.\label{fig:cont}}
\end{figure}%

\begin{figure}[h!]
\centering
\begin{subfigure}{\textwidth}
\centering
    \includegraphics[width=\textwidth]{img/discr_comparison_035.png}
    \caption{$\grinder$ vs. $\textsc{Exp3}$ for a predefined action set.}
    \label{fig:discr-035}
\end{subfigure}\\
\begin{subfigure}{\textwidth}
\centering
    \includegraphics[width=\textwidth]{img/cont_delta_comparison_035.png}
    \caption{$\grinder$ vs. $\textsc{Exp3}$ for a continuous action set.}
    \label{fig:cont-035}
\end{subfigure}\\
\caption{Regret Performance of $\grinder$ vs $\textsc{Exp3}$ for $\delta = 0.35$; in all cases, $\grinder$ converges faster.}\label{fig:app-035}
\end{figure}

\paragraph{Results.} In Figure~\ref{fig:discr} we present the results for the predefined action set as a way to measure experimentally the performance of our approximation oracle compared to the precise one. In summary, we see that both with the use of a precise oracle and with the use of an approximation one for every $\delta$, and for every $p$ our algorithm performs better than $\textsc{Exp3}$. Interestingly, the approximation oracle follows very closely the performance of the precise one. Since it is not generally possible to compute the best-fixed action in hindsight in the continuous case, we resort to depicting the \emph{cumulative losses} of the two algorithms. As for the fully continuous action set, we see in Figure~\ref{fig:cont} that for the more realistic cases of $p = 0.6, 0.8$, $\grinder$'s regret clearly outperforms that of $\textsc{Exp3}$. It is worth noting here that we have run $\grinder$ with a relatively simple logistic regression oracle; for more advanced oracles, the results would be strengthened. The latter is also the reason that we see that in some cases with a majority of attackers ($p = 0.4$), we perform comparably to $\textsc{Exp3}$, which, however, is bound to incur linear regret in the worst case, as we have reasoned about in Section~\ref{sec:regret-notions} (see Theorem~\ref{thm:incomp-sr-ext}). We also include the results of our simulations for $\delta = 0.35$ in Figure~\ref{fig:app-035} and $\delta = 0.7$ in Figure~\ref{fig:app-070} both for the predefined action set and the continuous one. 


\begin{figure}[h!]
\centering
\begin{subfigure}{\textwidth}
\centering
    \includegraphics[width=\textwidth]{img/discr_comparison_070.png}
    \caption{$\grinder$ vs. $\textsc{Exp3}$ for a predefined action set.}
    \label{fig:discr-070}
\end{subfigure}\\
\begin{subfigure}{\textwidth}
\centering
    \includegraphics[width=\textwidth]{img/cont_delta_comparison_070.png}
    \caption{$\grinder$ vs. $\textsc{Exp3}$ for a continuous action set.}
    \label{fig:cont-070}
\end{subfigure}\\
\caption{Regret Performance of $\grinder$ vs $\textsc{Exp3}$ for $\delta = 0.70$; in all cases, $\grinder$ converges faster.}\label{fig:app-070}
\end{figure}



==> 6-conclusion.tex <==
\section{Discussion and Open Questions}\label{sec:concl}

In this paper, we have studied online learning against $\delta$-bounded, strategic agents in classification settings, for which we provided the $\grinder$ algorithm. We complemented our theoretical analysis with simulations, showing first the benefits of our algorithm with a precise oracle, and second, that there are approximation oracles that perform comparably well. 

There is a number of interesting questions stemming from our work. On a technical level, an interesting research direction is to provide both theoretical results regarding the Stackelberg regret experienced by the learner for the case that she uses \emph{approximation} oracles (e.g., similar to the ones used in the simulations) and experimental ones for different variants of the agents' best-response oracles. In many natural settings (mostly the ones that are considered in the fairness community, as mentioned by \citet{BLRWW19}), the learner can only observe the labels of \emph{some} of the agents. This partial observability imposes an extra challenge, and cannot be handled by our framework currently. Moreover, our current analysis is based on the fact that the learner knows $\delta$ a priori, but no studies exist currently about an estimation of $\delta$. We believe that this can only be achieved through experiments with human subjects in as realistic conditions as possible. Finally, we do believe that the agents' real feature vectors are neither fully stochastic, nor fully adversarial. This model formulation is similar to the one considered in the recent line of works in the online learning literature on the best-of-both-worlds \citep{BS12,SS14,AC16,SL17} regret bounds. We believe it would be very interesting to provide theoretical bounds for the Stackelberg regret in such strategic classification settings. 

%


==> impact.tex <==
%
\section*{Broader Impact}

In this paper we put forth and study a model for strategic classification against real-life agents. We believe that when Machine Learning (ML) algorithms are deployed for real-life decision-making, the agents that we face (e.g., the human subjects that we wish to ``classify'') will not try to sabotage the decision-making algorithms, but they will try to manipulate them. The power and the ability to manipulate a decision-making rule is inherently tied to the learned outcome for the rule. Strategic ML aims to address these concerns with the construction of ML algorithms that are either \emph{strategyproof} (i.e., they provide no incentive to the agents to manipulate) or that are \emph{strategy-aware} (i.e., they are not affected too much by strategic manipulations). %


We think that since classification is a fundamental ML task, computer scientists together with economists should try to understand two key questions: 
\squishlist
\item[1.] What is the ``correct'' behavioral model to explain the agents' reports? 
\item[2.] How do we design ML algorithms that take this behavioral model into account, before deploying the algorithms for policy making?
\squishend

However, blindly optimizing predictive accuracy and the role of incentives in it, can have detrimental societal effects. For example, there have been works recently analyzing the disparate effects that strategic manipulation can have among different groups (\citep{HIV19,MMDH19}) when the agents' utility functions are similar to the ones considered by~\citet{HMPW16}. We believe that a next step for learning strategy-aware linear classifiers against \dBMR is to study whether there exist algorithms that concurrently satisfy the no-regret property and provide better societal guarantees. 



==> old_sec1.tex <==

%

%

\paragraph{Protocol.}Let $d \in \bbN$ denote the dimension of the problem and $\calA \subseteq [-1,+1]^{d+1}$ the learner's action space\footnote{This is without loss of generality, as the normal vector of any hyperplane could be normalized to lie in $[-1,1]^{d+1}$.}. Actions $\alpha \in \calA$ correspond to hyperplanes, written in terms of their normal vectors, and  without loss of generality, we assume that the $(d+1)$-th coordinate encodes information about the intercept. Let $\calX \subseteq ([0,1]^d,1)$ the feature vector space, where by $([0,1]^d,1)$ we denote the set of all $(d+1)$-dimensional vectors with values in $[0,1]$ in the first $d$ dimensions and value $1$ in the $(d+1)$-th. Let $h^{\star}: \calX \to \{-1,1\}$ be an \emph{ideal} classifier, \emph{not necessarily belonging in $\calA$}, which we assume makes \emph{no} error in identifying the labels of the feature vectors that it is given as input\footnote{One could think of $h^{\star}(\vx)$ as the label that a human verifier would assign to feature vector $\vx$.}. We use the contruction of $h^{\star}$ solely as a modeling tool, and our results assume no access to it. For a feature vector $\vu$, we refer to $h^{\star}(\vu)$ as its \emph{true} label. Formally, the protocol of the interaction of the learner with the agents (which repeats for all timesteps $t \in [T]$) is given in Protocol~\ref{protocol}. 
%
%
%
%
%
%
%
%
%
%
%
%
\begin{algorithm}[htbp]
\DontPrintSemicolon
\SetAlgorithmName{Protocol}{Protocol}
\SetAlgoLined
\caption{Learner-Agent Interaction at Round $t$}\label{protocol}
Nature adversarially selects feature vector $\vx_t \in \calX \subseteq ([0,1]^d, 1)$.\;
The learner chooses action $\alpha_t \in \calA$, and commits to it. \;
An agent observes $\alpha_t$ and $\sigma_t = (\vx_t, y_t)$, where $y_t = h^{\star}(\vx_t)$.\; 
The agent reports feature vector $\vz_t\left( \alpha_t; \sigma_t \right) \in \calX$ (potentially, $\vz_t\left( \alpha_t; \sigma_t \right) \neq \vx_t$). \label{step:protocol-4}\;
The learner observes $\left(\vz_t(\alpha_t; \sigma_t), \hat{y}_t\right)$, where $\hat{y}_t = h^{\star}\left(\vz_t\left( \alpha_t; \sigma_t \right)\right)$, and incurs binary classification loss $\ell\left(\alpha_t, \vz_t\left( \alpha_t; \sigma_t \right)\right) = \1 \left\{ \sgn\left(\hat{y}_t \cdot \langle \alpha_t, \vz_t\left( \alpha_t; \sigma_t \right) \rangle \right) = -1 \right\}$. \;
\end{algorithm}%

\paragraph{Agents' Behavior (Step~\ref{step:protocol-4}): Myopically Rational and $\delta$-Bounded.}We assume that when the agent reports $\mathbf{z}_t(\alpha_t; \sigma_t)$, instead of his true (i.e., assigned by nature) feature vector $\vx_t$, he gets \emph{utility} which is comprised by two parts; first, a \emph{value} $v_t( \alpha_t, \mathbf{z}_t(\alpha_t; \sigma_t)) \geq 0$, and second, a cost $c_t (\alpha_t, \mathbf{z}_t(\alpha_t; \sigma_t )) \geq 0$. Altogether, the agent's utility for reporting $\mathbf{z}_t(\alpha_t; \sigma_t)$ is equal to: \[{u_t( \alpha_t, \mathbf{z}_t(\alpha_t; \sigma_t))} = v_t( \alpha_t, \mathbf{z}_t(\alpha_t; \sigma_t)) - c(\alpha_t, \vz_t(\alpha_t; \sigma_t))\]As we observe, for a broad class\footnote{Notable members of this class are the rather natural value function: ${v_t (\alpha, \vz_t(\alpha;\sigma_t))} = \delta \cdot \1 \{\langle \alpha, \vz(\alpha; \sigma_t) \rangle \geq 0\}$ (which provides a value of $\delta$ to the agent if his reported feature vector is in the positive halfspace of $\alpha$) and the cost function: ${c_t(\alpha, \vz_t(\alpha;\sigma_t))} = \|\vx_t - \vz_t(\alpha;\sigma_t)\|_2$ (which models how far the original feature vector was from the ultimately reported one).} of value and cost functions this implies that the agent's best response lies in a ball of radius $\delta \in (0,1]$ (for appropriately tuned $\delta$). Importantly, the learner does \emph{not} know the specific value and cost functions. What she does know is the \emph{general form} of the utility function (i.e., value $-$ cost) and the scalar $\delta$ (or its upper bound). In terms of behavior, the agents are \emph{myopically rational}: in Step~\ref{step:protocol-4} of Protocol~\ref{protocol} they report a feauture vector maximizing their underlying utility $\vr_t\left( \alpha_t; \sigma_t \right) = \arg \max_{\mathbf{z}_t \in \calX; \sigma_t} u_t\left( \alpha_t, \mathbf{z}_t (\alpha_t; \sigma_t)\right)$\footnote{When clear from context, we write $\vr_t(\alpha_t)$ instead of $\vr_t\left( \alpha_t; \sigma_t \right)$, in order to simplify notation.}. Due to this, we refer to the agents as being \emph{myopically rational and $\delta$-bounded}. We remark here that if the agents were \emph{adversarial} instead of strategic, they would report $\max_{\|\vz - \vx_t \| \leq \delta} \ell(\alpha, \vz)$. 

Motivated by the spam emails setting, we assume that the agents derive no value if, by manipulating their feature vector from $\vx_t$ to $\vz_t\left( \alpha_t; \sigma_t \right)$, they also change $y_t$. Indeed, a spammer ($y_t = -1$) wishes to fool the learner's classifier, without actually having to change their email to be a non-spam one ($\hat{y}_t = 1$). So since for symmetric losses (e.g., $0-1$ as we use), agents derive no value when $\hat{y}_t \neq y_t$, then by observing $\hat{y}_t$, the learner essentially observes $y_t$. We, hence, drop the notation $\hat{y}_t$ and only use $y_t$ for the rest of the paper. %

\paragraph{Model Comparison with \citet{drsww18}.}Prior to our work, \citet{drsww18} studied online learning in strategic classification settings. Their work is orthogonal to ours in one key aspect: they find the appropriate conditions which can guarantee that the best-response of an agent, written as a function of the learner's action, is concave. As a result, in their model the learner's loss function becomes \emph{convex} and well known online convex optimization algorithms could be applied (e.g., \citep{FKM05,BLE17}) in conjunction with the mixture feedback that the learner receives. The foundation of our work, however, is to provide solutions (potentially of independent interest) for a setting where standard online learning algorithms could not be applied. Additionally, our work focuses on binary loss functions for the learner, while being able to accommodate even $0-1$ value functions, thus answering the open questions posed by \citet{drsww18}. More broadly, our work is situated at the interface of three research areas: learning using data from strategic data sources, Stackelberg games and multi-armed bandits. Due to space constraints, we defer the extended discussion on the related work to Appendix~\ref{sec:rel-work}.%


\paragraph{Solution Concept.} The goal of the learner is to minimize her Stackelberg regret. In the language of strategic classification, we compare the loss of the learner's deployed linear classifiers against the loss of the best-fixed linear classifier in hindsight, had the learner given the agents the opportunity to best-respond to it. Formal definitions are provided in Section~\ref{sec:regret-notions}.

\subsection{Our Results and Techniques}\label{subsec:res-tech}

\paragraph{Incompatibility Between External and Stackelberg Regret.}But why would one consider the arguably weirder notion of Stackelberg regret in the first place, when there are several works in online learning reducing the standard notion of external regret to other notions? Our first result answers this question; starkingly, we show that despite our intuition that there is a clear hierarchy between external and Stackelberg regret, the two are \emph{strongly incompatible} for strategic classification settings of interest; i.e., there exist strategic classification settings against myopically rational $\delta$-bounded agents, where \emph{any} online learning algorithm achieving \emph{sublinear} Stackelberg regret incurs \emph{linear} external regret, and \emph{any} online learning algorithm achieving \emph{sublinear} external regret suffers from \emph{linear} Stackelberg regret (Theorem~\ref{thm:incomp-sr-ext}). 

As a result, for online learning in strategic classification settings against myopically rational $\delta$-bounded agents, readily applying algorithms minimizing the external regret is not helpful. Even worse, the agent best responds to the learner's actions according to an \emph{unknown} utility function, and in the worst case the loss function of the learner as a function of her action is \emph{not even} Lipschitz%
\footnote{For learner's action $\alpha \in \calA$ let the agent's valuation and cost functions be $v(\alpha, \vz(\alpha; \sigma)) = \delta \1 \{ \langle \alpha, \vz(\alpha; \sigma) \rangle \geq 0\}\cdot \1\{\hat{y} = y\}$ and $c(\alpha,\vz(\alpha;\sigma)) = (\vx - \vz(\alpha;\sigma))^2$ respectively. The learner's loss function (i.e., $\ell(\alpha', \vz(\alpha';\sigma)) = \1 \{\sgn(\hat{y}\cdot \langle \alpha', \vz(\alpha';\sigma) \rangle ) = - 1\}, \alpha' \in \calA$) is clearly not Lipschitz.}. In light of this, a novel approach is required for the problem of learning to classify against strategic agents. Our approach is based on the fact that for such settings, despite the fact that the learner's loss function does not belong to any specific function family, we can still infer the loss of the learner for some actions against the best-responses of the agents for these actions, i.e., $\ell(\alpha,\vr_t(\alpha))$. Before outlining who to do this, we remark here that inferring the loss $\ell(\alpha, \vr_t(\alpha_t))$ is a very easy task. However, it can turn out to be rather useless, due to the strong incompatibility between the external and the Stackelberg regret.

\begin{wrapfigure}{R}{0.35\textwidth}
    \centering
    \begin{tikzpicture}[line cap=round,line join=round,>=latex',x=20.0cm,y=20.0cm, scale=0.4]
        %
        \draw [color=white, xstep=2.0cm,ystep=2.0cm] (-0.1,-0.1) grid (0.5,0.4);
        \draw[->,color=black] (-0.1,0.) -- (0.5,0.); %
        \foreach \x in {-0.1, 0.1, 0.2, 0.3, 0.4}
        \draw[shift={(\x,0)},color=black] (0pt,2pt) -- (0pt,-2pt) node[below] {};
        \draw[->,color=black] (0.,-0.1) -- (0.,0.4); %
        \foreach \y in {-0.1, 0.1, 0.2, 0.3}
        \draw[shift={(0,\y)},color=black] (2pt,0pt) -- (-2pt,0pt) node[left] {};
        \draw[color=black] (0pt,-10pt) node[right] {};
        \draw [line width=1pt,color=red] (-0.05,0.35) -- (0.35,-0.1);
        \draw [line width=1pt, dashed]      (-0.05, 0.33) -- (0.44, 0.33); 
        \draw [line width=1pt, dashed]      (-0.07, -0.1) -- (0.05, 0.37); 
        \draw [line width=1pt, color=blue, dotted] (0.2,0.05) circle (2.cm);
        \draw [line width=1pt,color=green!50!black] (0.24,0.09) circle (4.cm);
        \draw [->,color=green!50!black] (0.24,0.085) -- (0.435,0.13);
        \draw [->,color=blue] (0.2,0.05) -- (0.14,-0.028);
        \begin{footnotesize}
        \draw[color=red] (-0.03,0.3) node {$\alpha$};
        \draw[color=black] (0.47, 0.33) node {$\beta$};
        \draw[color=black] (0.07, 0.37) node {$\gamma$};
        \draw[color=black]  (0.5, -0.02) node {$x$};
        \draw[color=black]  (-0.02, 0.4) node {$y$};
        \draw [fill=blue] (0.2,0.05) circle (2pt);
        \draw[color=blue] (0.22,0.02) node {$\vx_t$};
        \draw[color=blue] (0.15,0.11) node {};
        \draw [fill=green!50!black] (0.24,0.085) circle (2pt);
        \draw[color=green!50!black] (0.225,0.11) node {$\vr_t(\alpha)$};
        \draw[color=green!50!black] (0.14,0.24) node {};
        \draw[color=green!50!black] (0.35,0.08) node {$2\delta$};
        \draw[color=blue] (0.16,0.03) node {$\delta$};
        \end{footnotesize}
        \end{tikzpicture}
    \caption{Agent's action space: $\alpha, \beta, \gamma$ are the learner's actions, $\vx_t$ is the agent's true feature vector and $\vr_t(\alpha)$ his misreport against $\alpha$.}\label{fig:2delta-ball}
\end{wrapfigure}
\paragraph{Inferring $\ell(\alpha,\vr_t(\alpha))$ Without Observing $\vx_t$.}Our results are enabled by thinking of the learner's and the agent's action spaces as dual ones. We focus on the agent's action space first. Because $\calX$ is a bounded feature vector space, the utility functions of the agents satisfy a nice $\delta$-boundedness property (for an appropriately tuned $\delta$, which is instance specific)\footnote{Our presented Stackelberg regret bounds are \emph{tighter} and \emph{more informative} for smaller values of $\delta$.}; i.e., given feature vector $\vx_t$ the agent can only misreport within the ball of radius $\delta$ centered around $\vx_t$, pictorially shown as the purple, dotted circle for $d=2$ in Figure~\ref{fig:2delta-ball} and henceforth denoted by $\calB_\delta(\vx_t)$. Since the learner observes $\vr_t(\alpha)$ and knows that the agent misreports in a ball of radius $\delta$ around $\vx_t$ (which remains unknown to her), the learner knows that in the worst case the agent's $\vx_t$ is found within the ball of radius $\delta$ centered at $\vr_t(\alpha)$. Note that since $\vr_t(\alpha)$ can be at the boundary of $\calB_\delta(\vx_t)$, the set of all of the agent's possible misreports against any committed action $\alpha'$ from the learner $\vr_t\left(\alpha' \right)$ is the \emph{augmented} $2\delta$ ball drawn with the green solid line in Figure~\ref{fig:2delta-ball}. This means that, since $y_t$ is also observed by the learner, she can infer her loss $\ell(\alpha', \vr_t(\alpha'))$ for \emph{any} action $\alpha'$ that has $\calB_{2\delta}(\vr_t(\alpha))$ \emph{fully} in an open halfspace (for example, actions $\beta,\gamma$ in Figure~\ref{fig:2delta-ball}). 


In the learner's action space, where actions $\alpha, \beta, \gamma$ are just multidimensional \emph{points}, the aforementioned observation has a nice mathematical translation. An action $\gamma$ has $\calB_{2\delta}(\vr_t(\alpha))$ fully in one of its open halfspaces, if its distance from $\vr_t(\alpha)$ is more than $2\delta$. Alternatively, for all actions $\alpha'$ such that: \[\frac{\abs*{\langle \alpha', \vr_t(\alpha) \rangle}}{\|\alpha'\|_2} \leq 2\delta \Leftrightarrow \abs*{\langle \alpha', \vr_t(\alpha) \rangle} \leq 4\sqrt{d} \delta\]where the last inequality comes from the fact that $\calA \subseteq [-1,1]^{d+1}$, the learner cannot infer the loss $\ell(\alpha', \vr_t(\alpha'))$, unless she has some prior information about the agent's utility function. But for all other actions $\gamma$ in $\calA$, the learner can compute her loss \emph{precisely}, due to the fact that she always knows that $\vr_t(\gamma)$ lies somewhere within $\calB_{2\delta}(\vr_t(\alpha))$. From that, we derive that the learner can discretize her action space into the following \emph{polytopes}: upper polytopes $\calP_t^u$, containing actions $\vw \in \calA$ such that $\langle \vw, \vr_t(\alpha) \rangle \geq 4\sqrt{d} \delta$ and lower polytopes $\calP_t^l$, containing actions $\vw' \in \calA$ such that $\langle \vw', \vr_t(\alpha) \rangle \leq -4 \sqrt{d} \delta$. The distinction into the two sets is helpful as one of them always assigns label $+1$ to the agent's best-response, and the other always assigns label $-1$. Clearly, the size of $\calP_t^u$ and $\calP_t^l$ depends on how big $\delta$ is. 

\paragraph{Stackelberg Regret Upper and Lower Bounds.}The $\grinder$ algorithm uses the above as follows: It maintains a sequence of nested polytopes at all timesteps, and adaptively keeps adding new polytopes to the learner's action space (i.e., ``grinding'' it) according to the responses received from the agents. We provide two regret bounds for $\grinder$: the first one is tighter (Theorem~\ref{thm:regr-grind}), while the latter is much more intuitive (Corollary~\ref{cor:sr-loose}). The looser, more intuitive upper bound is that $\grinder$ incurs Stackelberg regret: $$\calR(T) \leq \calO \left(\sqrt{\log \left(T \frac{\lambda(\calA)}{\lambda(\up)} \right)\cdot \log \left(\frac{\lambda(\calA)}{\lambda(\up)} \right)\cdot T} \right)$$where by $\up$ we denote the polytope with the smallest Lebesgue measure in the finest partition of the learner's action space, and {$\lambda(A)$} denotes the Lebesgue measure of measurable space $A$.  


Unfortunately, this upper bound depends heavily on quantity $\log (\lambda(\calA)/\lambda(\up))$, which is rather unsatisfactory, as there are sequences of labeled datapoints $\{\sigma_t\}_{t=1}^T$ where $\lambda(\up)$ becomes so small compared to $\lambda(\calA)$, that the upper bound on the Stackelberg regret of $\grinder$ becomes vacuous. That said, we prove that this dependence is (up to an extent) unavoidable (Theorem~\ref{thm:lb}) as the Stackelberg regret of learning a linear classifier against myopically rational $\delta$-bounded strategic agents is lower bounded by $\Omega\left(\sqrt{T \log \left(\frac{\lambda(\calA)}{\lambda(\up)} \right)}\right)$. Hence, the regret bound of $\grinder$ is nearly optimal.

Before we move on to the formal presentation of our results, we clarify the following: $\grinder$ assumes access to an \emph{in-oracle}, i.e., an oracle that computes the probability that each action $\alpha \in \calA$ will be updated by another action $\alpha' \in \calA$. To relax this assumption, we provide simulation results showing that our regret guarantees carry over for approximation oracles as well.

%




==> related_work.tex <==
\section{Further Related Work}\label{sec:rel-work}

In this section we discuss the connections that our work has with the literature around three main areas: learning using data from strategic data sources, Stackelberg games and multi-armed bandits. We also outline some connections with the literature on learning halfspaces with malicious or bounded noise.

\paragraph{Learning using data from strategic sources.}Recently, there has been an increasing body of work studying machine learning algorithms that are trained on data controlled by \emph{strategic} agents. In this context, the two most studied machine learning tasks for which such algorithms are provided are \emph{classification}, and \emph{linear regression}. For linear regression, most of the works focus on the \emph{offline} setting where the agents hold as their manipulable information their \emph{dependent variables}, and they have either privacy concerns \citep{CIL15,CDP15}, or they wish to make the algorithm predict correctly on their input \citep{PP04,DFP10,CPPS18}. There is also a parallel line of work focused on the problem of competing algorithms in the context of strategic linear regression \citep{BPT17, BPT18}. Both stand in contrast to our model, which is inherently dynamic and online. The situation for the task of classification is similar; most of the existing works are written from the perspective of an \emph{offline} setting \citep{WC09,BS11,MAMR11,MPR12,HMPW16}, with the exception of \citep{drsww18}. Contrary to our setting, in the models used by \citet{MAMR11,MPR12} the \emph{feature vectors} of the agents are assumed to be publicly verifiable, while similarly to our setting in \citep{WC09,BS11,HMPW16,drsww18} the \emph{feature vectors} are the only manipulable piece of information that the agents possess. Our work, which assumes only knowledge of the general family of utility functions for the agents, differs from \citep{WC09,BS11,HMPW16}, as they consider a learner who knows either fully the strategic agents' utility function, or some prior distribution. A byproduct of this is that our solution concept is the one of Stackelberg regret, rather than the notions of Nash and Stackelberg Equilibria considered in \citep{WC09,BS11,HMPW16}.


Our work is most closely related to the work of \citet{drsww18}, who also studied online learning in strategic classification settings. However, their work is orthogonal to ours in one key aspect: they find the appropriate conditions which can guarantee that the best-response of an agent, written as a function of the learner's action, is concave. As a result, in their model the learner's loss function becomes \emph{convex} and well known online convex optimization algorithms could be applied (e.g., \citep{FKM05,BLE17}) in conjunction with the mixture feedback that the learner receives. The foundation of our work, however, is to provide solutions (potentially of independent interest) for a setting where standard online learning algorithms could not be applied. Additionally, our work focuses on binary loss functions for the learner, while being able to accommodate even $0-1$ value functions, thus answering the open questions posed by \citet{drsww18}.


Another line of research falling under the general umbrella of learning using data from strategic sources that our work is related to, is the research on \emph{learning from revealed preferences} (see e.g., \citep{BV06,ZR12,BDMUV14,ACDKR15,RUW16,JRRW16,RSUW17,BMM18}). Abstracting away from the specificities of each model, most of these works are centered around a buyer-seller problem with (potentially) combinatorial preferences, where buyers respond to the sellers' offers by revealing their preferences, rather than their actual value for a choice they made. Our revealed preferences model is centered around the problem of classification, and crucially, presents a lot less structure in the agents' and the learner's utility and loss functions respectively than what is usually assumed in the learning from revealed preferences literature. Finally, there has been recent interest in learning against no-regret learners \citep{BMSW18,DSS19,DSS19b}. Our setting differs from these works in that the agents that we consider are \emph{myopically} rational. 
%
\paragraph{Stackelberg Games.} Our work is also related to the Stackelberg games literature, which has mostly dealt with Stackelberg Security Games (SSGs). It is nearly impossible for us to survey the vast literature in SSGs, but we refer the interested reader to \citep{T11,SFAKT18} for overviews. There has also been work in learning theoretic problems related to SSGs (\citep{LCM09,MTS12,BHP14,BBHP15}). Out of these, the one most related to our work is the work of \citet{BBHP15}, who provide information theoretic sublinear Stackelberg regret\footnote{Even though the formal definition of Stackelberg regret was only later introduced by \citet{drsww18}.} algorithms for the learner. In SSGs the utilities of the agents and the learner have nice linearity properties, which are not present in the setting of online strategic classification that we consider. 


\paragraph{Multi-Armed Bandits.} Finally, our work is related to the vast literature in online learning with partial feedback (see \citep{BCB12,S19,LS19} for excellent overviews of the field). However, our strategic classification setting presents a unique form of feedback, which depends on the best-response of the agents to the learner's committed actions. For online learning Lipschitz functions in stochastic environments \citet{KSU08} and \citet{BMSS11} provided adaptive discretization algorithms which take advantage of the specifics of each problem instance, and performed ``better'' in ``good'' instances. The $\grinder$ algorithm is an adaptive discretization algorithm for a problem that is not at all stochastic, contrary to what has been the case in the works of \citet{KSU08,BMSS11}. Further, our work is related to the literature in online learning with feedback graphs \citep{NCBDK15,CHK16}. In fact, as we explain in Section~\ref{sec:grinding-algo}, if the learner were to be given a predefined set of actions instead of a continuous interval, one could almost straightforwardly apply the feedback graph results and guarantee sublinear Stackelberg regret. However, in our work, we are dealing with the infinite set of actions inside a continuous interval, which makes the application of previous results impossible. 

Finally, connecting learning from strategic sources and online learning for multi-armed bandits, \citet{BMSW19} studied a model where each arm is controlled by a strategic entity who chooses the amount of the reward that it will pass to the learner. In our model, the arms are not explicitly controlled by anybody.



\paragraph{Learning Halfspaces with Malicious or Bounded Noise.} Distantly related to our work is the problem of learning halfspaces with malicious or bounded noise (e.g., \citep{KLPS09,ABHU15,DGT19,DKM19}) in the offline setting. Our work has significant differences from these settings; we do not make \emph{any} distributional assumptions about $\{\vx_t\}_{t=1}^T$, our agents \emph{cannot} alter their $y_t$'s, and ultimately, they have \emph{agency} about what they misreport. What does seem to be a connection between our paper and this line of works can be seen in the lower bound; it is well known that if certain margin assumptions are not satisfied, then it is not possible to learn a linear separator in the offline setting. Our lower bound seems to provide the same interpretation, but for the online, strategic setting; indeed, one can easily create a sequence of $\{\vx_t\}_{t=1}^T$ with almost zero margin, such that $\lambda(\up) \to 0$.


